Generative Models for Learning from Crowds

In this paper, we propose generative probabilistic models for label aggregation. We use Gibbs sampling and a novel variational inference algorithm to perform the posterior inference. Empirical results show that our methods consistently outperform state-of-the-art methods.

==> model_f_idbla.tex <==
%IDBLA
\begin{tikzpicture}[x=1.7cm,y=1.8cm]
  
  %%%
  \node[obs] (L) {$L_{i,k}$};
  \node[latent, below=2.1 of L] (Q) {$Q_i$};
  \factor[left=1.2 of L, yshift=-1.5cm] {L-f1} {below:Multi} {} {};
  \factor[right=1.2 of L, yshift=-1.5cm] {L-f2} {below:Multi} {} {};
  \node[obs, left=0.7 of L-f1] (pi1) {$\bm{\pi}^{(k,h)}_{t}$};
  \node[latent, right=1.2 of L-f2] (pi2) {$\bm{\pi}^{(k,h)}_{t}$};
  \node[latent, above=0.6 of L] (T) {$T_i$};
  
  %Q
  \factor[right=1.0 of Q] {Q-f} {Multi} {} {};
  \node[latent, right=0.8 of Q-f] (beta) {$\bm{\beta}$};
  \factor[right=of beta] {b-f} {Dir} {} {};
  \node[const, right=0.3 of b-f] (gbeta) {$\bm{\gamma}_{\beta}$};
  \factoredge{gbeta}{b-f}{beta};
  \factoredge{beta}{Q-f}{Q};
  
  %T
  \factor[left=1.0 of T] {T-f} {Multi} {} {};
  \node[latent, left=1 of T-f] (alpha) {$\bm{\alpha}$};
  \factor[left=of alpha] {a-f} {Dir} {} {};
  \node[const, left=0.3 of a-f] (galpha) {$\bm{\gamma}_{\alpha}$};
  \factoredge{galpha}{a-f}{alpha};
  \factoredge{alpha}{T-f}{T};
  
  %pi
  \factor[above=of pi2] {pi-f} {left:Dir} {} {};
  \node[const, above=0.3 of pi-f] (psi) {$\bm{\psi}_{t}^{(k,h)}$};
  \factoredge{psi} {pi-f} {pi2};
  
  %L
  \gate {L-gate1} {(L-f1)(L-f1-caption)} {T,Q}
  \factoredge{pi1} {L-f1} {L};
  \gate {L-gate2} {(L-f2)(L-f2-caption)} {T,Q}
  \factoredge{pi2} {L-f2} {L};
  
  \vgate {L-vgate} %
  {(L-gate1)} {$Q_i \geq H-1$} %
  {(L-gate2)} {$Q_i < H-1$} %
  {Q} ; %
  
  \plate {plate1} { %
    (pi1)%
  } {$t=1,...,C$} ; %
  \plate {plate2} { %
    (plate1)%
  } {$h=H-1,H$} ; %
  
  \plate {plate3} { %
    (pi2)%
    (psi)
  } {$t=1,...,C$} ; %
  \plate {plate4} { %
    (plate3)%
  } {$h=1,...,H-2$} ; %
  \plate {plate5} {
    (plate2)
    (plate4)
    (L)
  } {$k=1,...,K$}
  \plate {plate6} {
    (T)
    (L)
    (Q)
    (L-vgate)
  } {$i=1,...,I$}
  
\end{tikzpicture}

==> model_idbla.tex <==
%IDBLA
\begin{tikzpicture}[x=1.7cm,y=1.8cm]
  
  %%%
  \node[obs] (L) {$L_{i,k}$};
  \factor[above=of L] {L-f} {Multi} {} {};
  \node[latent, left=of L-f] (pi) {$\bm{\pi}^{(k,h)}_{t}$};
  \node[latent, right=2 of L-f, xshift=-0.4cm, yshift=0.22cm] (Q) {$Q_i$};
  \node[latent, above=of L-f, xshift=2.0cm, yshift=-1.0cm] (T) {$T_i$};
  \factor[above=of pi] {pi-f} {left:Dir} {} {};
  \factor[above=of T] {T-f} {right:Multi} {} {};
  \factor[above=of Q] {Q-f} {left:Multi} {} {};
  \node[const, above=of pi-f, yshift=-0.5cm] (omega) {$\bm{\omega}^{(k,h)}_t$};
  \node[latent, above=of T-f, yshift=-0.5cm] (alpha) {$\bm{\alpha}$};
  \node[latent, above=of Q-f, yshift=-1.0cm] (beta) {$\bm{\beta}$};
  \factor[left=of alpha] {a-f} {left:Dir} {} {};
  \factor[above=of beta] {b-f} {right:Dir} {} {};
  \node[const, above=of a-f, yshift=-1.4cm] (galpha) {$\bm{\gamma}_{\alpha}$};
  \node[const, above=of b-f, yshift=-1.1cm] (gbeta) {$\bm{\gamma}_{\beta}$};
  
  %%%
  \factoredge{pi} {L-f} {L};
  \factoredge{omega} {pi-f} {pi};
  \factoredge{galpha} {a-f} {alpha};
  \factoredge{gbeta} {b-f} {beta};
  \factoredge{alpha} {T-f} {T};
  \factoredge{beta} {Q-f} {Q};
  
  \gate {L-gate} {(L-f)(L-f-caption)} {T,Q}
  
  \plate {plate1} { %
    (pi)(omega)%
  } {$t=1,...,C$}; %
  \plate {plate2} { %
    (pi)(omega)%
    (plate1)
  } {$h=1,...,H$}; %
  \plate {plate4} { %
    (L)(L-gate) %
    (T)(Q)%
  } {$i=1,...,I$}; %
  \plate {plate3} { %
    (L)(L-gate) %
    (pi)(omega)%
    (plate2)
    (plate4.south west)
  } {$k=1,...,K$}; %
  
\end{tikzpicture}

